Mismatched Data Detection in Massive MU-MIMO

We investigate mismatched data detection for massive multi-user (MU) multiple-input multiple-output (MIMO) wireless systems in which the prior distribution of the transmit signal used in the data detector differs from the true prior. In order to minimize the performance loss caused by the prior mismatch, we include a tuning stage into the recently proposed large-MIMO approximate message passing (LAMA) algorithm, which enables the development of data detectors with optimal as well as sub-optimal parameter tuning. We show that carefully-selected priors enable the design of simpler and computationally more efficient data detection algorithms compared to LAMA that uses the optimal prior, while achieving near-optimal error-rate performance. In particular, we demonstrate that a hardware-friendly approximation of the exact prior enables the design of low-complexity data detectors that achieve near individually-optimal performance. Furthermore, for Gaussian priors and uniform priors within a hypercube covering the quadrature amplitude modulation (QAM) constellation, our performance analysis recovers classical and recent results on linear and non-linear massive MU-MIMO data detection, respectively.

==> macros/delta_star.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 8.1.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
\begin{tikzpicture}

\begin{axis}[%
width=5.16317052165354in,
height=3.59478807824803in,
scale only axis,
xmin=0.5,
xmax=1,
xlabel={$\sigma{}^\text{2}$},
xmajorgrids,
ymin=-0.1,
ymax=0.02,
ylabel={$\text{MSE }\Psi\text{(}\sigma{}^\text{2}\text{,}\delta\text{)}$},
ymajorgrids,
legend style={draw=black,fill=white,legend cell align=left},
scaled y ticks = false,
y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,precision=2}
]
\addplot [color=blue,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.00847186823552865\\
0.51	-0.00601453905159377\\
0.52	-0.00370544732742462\\
0.53	-0.00154476341156906\\
0.54	0.000467627376738888\\
0.55	0.00233209087222286\\
0.56	0.00404921374335487\\
0.57	0.0056197763556024\\
0.58	0.0070447284855838\\
0.59	0.00832516758867108\\
0.6	0.00946231935404707\\
0.61	0.010457520309356\\
0.62	0.0113122022622594\\
0.63	0.0120278783886857\\
0.64	0.0126061307976336\\
0.65	0.0130485994203295\\
0.66	0.0133569720875105\\
0.67	0.0135329756729161\\
0.68	0.0135783681937844\\
0.69	0.0134949317705579\\
0.7	0.0132844663581388\\
0.71	0.0129487841701174\\
0.72	0.0124897047255125\\
0.73	0.0119090504547793\\
0.74	0.0112086428083547\\
0.75	0.0103902988167651\\
0.76	0.00945582805653367\\
0.77	0.0084070299807415\\
0.78	0.00724569157726995\\
0.79	0.00597358532146186\\
0.8	0.0045924673932799\\
0.81	0.003104076132037\\
0.82	0.00151013070445061\\
0.83	-0.000187670035805887\\
0.84	-0.00198764851672595\\
0.85	-0.0038881492624897\\
0.86	-0.00588753956984844\\
0.87	-0.00798421006078442\\
0.88	-0.0101765751244192\\
0.89	-0.0124630732598896\\
0.9	-0.0148421673307546\\
0.91	-0.0173123447404596\\
0.92	-0.0198721175374564\\
0.93	-0.0225200224577413\\
0.94	-0.0252546209118061\\
0.95	-0.0280744989223199\\
0.96	-0.0309782670182411\\
0.97	-0.0339645600904978\\
0.98	-0.037032037213876\\
0.99	-0.0401793814392991\\
1	-0.0434052995602611\\
};
\addlegendentry{$\delta\text{=0.48}$};

\addplot [color=black!50!green,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0187120376472885\\
0.51	-0.0165142361546856\\
0.52	-0.0144615838414366\\
0.53	-0.0125542475071614\\
0.54	-0.0107921148602765\\
0.55	-0.00917482768761513\\
0.56	-0.00770181154296512\\
0.57	-0.00637230231847263\\
0.58	-0.00518537002453257\\
0.59	-0.00413994006942631\\
0.6	-0.00323481229916234\\
0.61	-0.00246867803042228\\
0.62	-0.00184013528487104\\
0.63	-0.00134770241107862\\
0.64	-0.00098983026065036\\
0.65	-0.000764913067593964\\
0.66	-0.000671298164312661\\
0.67	-0.000707294653602974\\
0.68	-0.000871181143586086\\
0.69	-0.00116121264132862\\
0.7	-0.0015756266909891\\
0.71	-0.00211264883342677\\
0.72	-0.00277049745626901\\
0.73	-0.0035473880963619\\
0.74	-0.00444153725015284\\
0.75	-0.00545116574191751\\
0.76	-0.00657450169464413\\
0.77	-0.00780978314385727\\
0.78	-0.00915526033058989\\
0.79	-0.0106091977060686\\
0.8	-0.0121698756774135\\
0.81	-0.0138355921207137\\
0.82	-0.0156046636852255\\
0.83	-0.01747542691006\\
0.84	-0.0194462391726276\\
0.85	-0.0215154794861878\\
0.86	-0.0236815491621433\\
0.87	-0.0259428723511849\\
0.88	-0.0282978964759938\\
0.89	-0.0307450925669753\\
0.9	-0.0332829555113638\\
0.91	-0.0359100042250333\\
0.92	-0.0386247817554261\\
0.93	-0.0414258553232051\\
0.94	-0.0443118163094768\\
0.95	-0.0472812801947716\\
0.96	-0.050332886455361\\
0.97	-0.0534652984219457\\
0.98	-0.0566772031052537\\
0.99	-0.0599673109926471\\
1	-0.0633343558194223\\
};
\addlegendentry{$\delta\text{=0.49}$};

\addplot [color=red,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0285342409606091\\
0.51	-0.0265853741923451\\
0.52	-0.0247786943752848\\
0.53	-0.0231143649049744\\
0.54	-0.0215922757814954\\
0.55	-0.0202120761021536\\
0.56	-0.0189732031441291\\
0.57	-0.0178749083936059\\
0.58	-0.0169162808403585\\
0.59	-0.0160962678231115\\
0.6	-0.015413693680812\\
0.61	-0.0148672764379647\\
0.62	-0.0144556427280369\\
0.63	-0.0141773411373831\\
0.64	-0.0140308541328821\\
0.65	-0.0140146087192757\\
0.66	-0.0141269859568777\\
0.67	-0.0143663294565907\\
0.68	-0.0147309529569823\\
0.69	-0.0152191470772199\\
0.7	-0.0158291853299485\\
0.71	-0.0165593294694794\\
0.72	-0.0174078342428757\\
0.73	-0.0183729516045994\\
0.74	-0.0194529344491293\\
0.75	-0.0206460399104498\\
0.76	-0.0219505322723045\\
0.77	-0.0233646855286765\\
0.78	-0.0248867856299656\\
0.79	-0.0265151324467612\\
0.8	-0.0282480414799152\\
0.81	-0.03008384534274\\
0.82	-0.0320208950385883\\
0.83	-0.0340575610547527\\
0.84	-0.0361922342915535\\
0.85	-0.0384233268436126\\
0.86	-0.0407492726486302\\
0.87	-0.0431685280174872\\
0.88	-0.0456795720581163\\
0.89	-0.0482809070043839\\
0.9	-0.0509710584601116\\
0.91	-0.0537485755673797\\
0.92	-0.0566120311073562\\
0.93	-0.0595600215410989\\
0.94	-0.0625911669970385\\
0.95	-0.0657041112112049\\
0.96	-0.0688975214256599\\
0.97	-0.0721700882500693\\
0.98	-0.0755205254908607\\
0.99	-0.0789475699519808\\
1	-0.0824499812108627\\
};
\addlegendentry{$\delta\text{=0.50}$};

\end{axis}
\end{tikzpicture}%
